All Cyclic Group Facets Inject

We give a variant of Basu-Hildebrand-Molinaro's approximation theorem for continuous minimal valid functions for Gomory-Johnson's infinite group problem by piecewise linear two-slope extreme functions [Minimal cut-generating functions are nearly extreme, IPCO 2016]. Our theorem is for piecewise linear minimal valid functions that have only rational breakpoints (in $1/q\,\mathbb{Z}$ for some $q\in \mathbb{N}$) and that take rational values at the breakpoints. In contrast to Basu et al.'s construction, our construction preserves all function values on $1/q\,\mathbb{Z}$. As a corollary, we obtain that every extreme function for the finite group problem on $1/q\,\mathbb{Z}$ is the restriction of a continuous piecewise linear two-slope extreme function for the infinite group problem with breakpoints on a refinement $1/(Mq)\,\mathbb{Z}$ for some $M\in \mathbb{N}$. In combination with Gomory's master theorem [Some Polyhedra related to Combinatorial Problems, Lin. Alg. Appl. 2 (1969), 451-558], this shows that the infinite group problem is the correct master problem for facets (extreme functions) of 1-row group relaxations.

==> Makefile-injective <==
# -*- Makefile -*-
LATEX=latex
PDFLATEX=pdflatex
FIG2DEV=fig2dev
BIBTEX=bibtex

FIGURESDIRPREFIX=

MAINTEXFILE=two_slope_fill_in_extreme

all: $(MAINTEXFILE).pdf

%.pstex_t: %.fig #Makefile
	$(FIG2DEV) -L pstex_t -p $*.pstex $< $@

%.pstex: %.fig #Makefile
	$(FIG2DEV) -L pstex $< $@

%.pdftex_t: %.fig #Makefile
	$(FIG2DEV) -L pdftex_t -p $*.pdf $< $@

%.pdf: %.fig #Makefile
	$(FIG2DEV) -L pdftex $< $@

INJECTIVE_GRAPHICS_SOURCES=

INJECTIVE_GENERATED_GRAPHICS=$(INJECTIVE_GRAPHICS_SOURCES:%.fig=$(FIGURESDIRPREFIX)%.pdftex_t) $(INJECTIVE_GRAPHICS_SOURCES:%.fig=$(FIGURESDIRPREFIX)%.pdf) 

#$(INJECTIVE_GRAPHICS_SOURCES:%.fig=%.pstex_t) $(INJECTIVE_GRAPHICS_SOURCES:%.fig=%.pstex)

INJECTIVE_SOURCES=Makefile-injective $(MAINTEXFILE).tex $(INJECTIVE_GRAPHICS_SOURCES:%.fig=$(FIGURESDIRPREFIX)%.fig) \
	sage-commands.tex 

INJECTIVE_STYLES = 

## copied these files from their source:
## $ (cd ~/Dropbox/yuan-group-relaxation-sage-code/ && tar cf - $files) | tar xvf -
INJECTIVE_GRAPHICS=$(INJECTIVE_GENERATED_GRAPHICS)							\
	funcgraphs/bhk_irrational.pdf									\
	graphics/case_a.pdf										\
	graphics/case_aprime.pdf									\
	graphics/case_b.pdf										\
	graphics/case_bprime.pdf									\
	graphics/counterexample-to-thm-82-left.png							\
	graphics/counterexample-to-thm-82-right.png							\
	graphics/example7slopecoarse2-inj_2_slope_fill_in_diagram.png					\
	graphics/example7slopecoarse2-sym_2_slope_fill_in_diagram.png					\
	graphics/lift_until_extreme_only_works_with_strict_subset_L-inj_2_slope_fill_in_diagram.png	\
	graphics/lift_until_extreme_only_works_with_strict_subset_L-sym_2_slope_fill_in_diagram.png	\
	graphics/minimal_has_uncovered_breakpoints-inj_2_slope_fill_in_diagram.png			\
	graphics/minimal_has_uncovered_breakpoints-sym_2_slope_fill_in_diagram.png			\
	graphics/minimal_has_uncovered_interval_order_16-inj_2_slope_fill_in_diagram.png		\
	graphics/minimal_has_uncovered_interval_order_16-sym_2_slope_fill_in_diagram.png		\
	graphics/minimal_has_uncovered_interval_order_8-inj_2_slope_fill_in_diagram.png			\
	graphics/minimal_has_uncovered_interval_order_8-sym_2_slope_fill_in_diagram.png			\
	graphics/not_extreme_1-inj_2_slope_fill_in_diagram.png						\
	graphics/not_extreme_1-sym_2_slope_fill_in_diagram.png

# copy-graphics-from-dropbox:
# 	(cd $$HOME/Dropbox/yuan-group-relaxation-sage-code/ && tar cf - $(INJECTIVE_GRAPHICS)) | tar xvf -

BIB=../../bib/MLFCB_bib.bib

.PHONY: figures

figures: $(INJECTIVE_GRAPHICS) 

$(MAINTEXFILE).pdf: $(MAINTEXFILE).tex $(INJECTIVE_GRAPHICS) $(BIB)
	$(PDFLATEX) -halt-on-error "$<"
	$(BIBTEX) $(MAINTEXFILE)
	$(PDFLATEX) -halt-on-error "$<"
	$(PDFLATEX) -halt-on-error "$<"

INJECTIVE_SOURCES_AND_MORE=$(INJECTIVE_SOURCES) $(INJECTIVE_GRAPHICS) $(INJECTIVE_STYLES)

.PHONY: arxiv
arxiv:
	COPYFILE_DISABLE=true tar -cf $(CURDIR)/$(MAINTEXFILE).tar	\
		$(MAINTEXFILE).bbl					\
		$(INJECTIVE_SOURCES)					\
		$(INJECTIVE_GRAPHICS)					\
		$(INJECTIVE_STYLES)
	rm -f $(MAINTEXFILE).tar.gz
	gzip $(MAINTEXFILE).tar

check-arxiv: arxiv
	rm -Rf t
	(mkdir t && cd t && tar xf ../$(MAINTEXFILE).tar.gz && ( $(PDFLATEX) -halt-on-error $(MAINTEXFILE) ; $(PDFLATEX) -halt-on-error $(MAINTEXFILE)))
	@echo "****************************************************"
	@echo "***** Check PDF in t/$(MAINTEXFILE).pdf"
	@echo "***** Then upload $(MAINTEXFILE).tar.gz to arXiv.org"


### -t CTRADITIONAL .... also nice
### -t BOLD

diff:
	latexdiff --preamble=latexdiff-preamble.tex --append-safecmd="DIFFPROTECT" --math-markup=2 two_slope_fill_in_extreme-MOR-submitted.tex two_slope_fill_in_extreme.tex > two_slope_fill_in_extreme-diff.tex
	cp two_slope_fill_in_extreme.bbl two_slope_fill_in_extreme-diff.bbl
	$(PDFLATEX) -halt-on-error two_slope_fill_in_extreme-diff
	$(PDFLATEX) -halt-on-error --synctex=1 two_slope_fill_in_extreme-diff

